Planimation

Planimation is a modular and extensible open source framework to visualise sequential solutions of planning problems specified in PDDL. We introduce a preliminary declarative PDDL-like animation profile specification, expressive enough to synthesise animations of arbitrary initial states and goals of a benchmark with just a single profile.

==> macros.tex <==
% % Environments and Theorems
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}{Example}

%%%%%%%%%%%%%%%%%%%%%%%%%% General Math

\newcommand{\A}{\mathcal{A}} \newcommand{\B}{\mathcal{B}}
\newcommand{\C}{\mathcal{C}} \newcommand{\D}{\mathcal{D}}
\newcommand{\E}{\mathcal{E}} \newcommand{\F}{\mathcal{F}}
\newcommand{\G}{\mathcal{G}} \renewcommand{\H}{\mathcal{H}}
\newcommand{\I}{\mathcal{I}} \newcommand{\J}{\mathcal{J}}
\newcommand{\K}{\mathcal{K}} \renewcommand{\L}{\mathcal{L}}
\newcommand{\M}{\mathcal{M}} \newcommand{\N}{\mathcal{N}}
\renewcommand{\O}{\mathcal{O}} \renewcommand{\P}{\mathcal{P}}
\newcommand{\Q}{\mathcal{Q}} \newcommand{\R}{\mathcal{R}}
\renewcommand{\S}{\mathcal{S}} \newcommand{\T}{\mathcal{T}}
\newcommand{\U}{\mathcal{U}} 
%\newcommand{\V}{\mathcal{V}}
\newcommand{\W}{\mathcal{W}} \newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}} \newcommand{\Z}{\mathcal{Z}}

\newcommand{\BE}{{\mathcal{B}, \mathcal{E}}} 

\newcommand{\TAU}{\mathcal{T}} 

\newcommand{\set}[1]{\{#1\}}                      % set
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\card}[1]{|{#1}|}                     % cardinality of a set
\newcommand{\Card}[1]{\left| #1\right|}
\newcommand{\sub}[1]{[#1]}
\newcommand{\tup}[1]{\langle #1\rangle}            % tuple
\newcommand{\Tup}[1]{\left\langle #1\right\rangle}

\newcommand{\pv}[1]{#1^{b}}
\newcommand{\sv}[1]{#1^{d}}

\newcommand{\hpp}{ \langle \pv{X},\sv{X},D,s_0,A,G,C \rangle }


% % % Names of things, acronyms, software, etc.
\newcommand{\propername}[1]{\text{\textsf{\small #1}}\xspace}

\newcommand{\PDDL}{\textsc{pddl}}
\newcommand{\PDDLplus}{\textsc{pddl}$+$}
\newcommand{\PDDLPlus}{\textsc{pddl}$+$}
\newcommand{\FPDDL}{$\smallint$-\textsc{pddl}$+$}
\newcommand{\ADL}{\textsc{adl}}
\newcommand{\FS}{\propername{FS}}
\newcommand{\FSTRIPS}{FSTRIPS}
\newcommand{\SMT}{\textsc{Smt}}
\newcommand{\SAT}{\textsc{Sat}}
\newcommand{\CP}{\textsc{Cp}}
\newcommand{\FMSMT}{\propername{FM-SMT}}
\newcommand{\HSHP}{\propername{HSHP}}
\newcommand{\CNF}{\propername{CNF}}
\newcommand{\Zthree}{\propername{Z3}}
\newcommand{\MathSat}{\propername{MathSAT}}
\newcommand{\LpSat}{\propername{LPSAT}}
\newcommand{\TmLpSat}{\propername{TM-LPSAT}}
\newcommand{\Colin}{\propername{COLIN}}
\newcommand{\PSR}{\textsc{Psr}}
\newcommand{\HBW}{\textsc{Hbw}}
\newcommand{\FF}{\propername{FF}}
\newcommand{\MetricFF}{\propername{MetricFF}}
\newcommand{\FSZero}{\propername{FS0}}
\newcommand{\FSPlus}{\propername{FS+}}
\newcommand{\LTI}{\textsc{Lti}}
\newcommand{\HA}{\textsc{Ha}}
\newcommand{\UPMurphi}{\propername{UPMurphi}}
\newcommand{\Dino}{\propername{DiNo}}
\newcommand{\dreal}{\propername{dReal}}
\newcommand{\Convoys}{\textsc{Convoys}}
\newcommand{\ENHSP}{\propername{ENHSP}}

\newcommand{\Kongming}{\propername{Kongming}}
\newcommand{\GraphPlan}{\propername{GraphPlan}}
\newcommand{\SpaceEx}{\propername{SpaceEx}}
\newcommand{\ode}{\textsc{ode}}
\newcommand{\blind}{\textsc{Brfs}}
\newcommand{\uct}{\textsc{Uct}}
\newcommand{\iwk}{\textsc{IW}($k$)}
\newcommand{\PNE}{\propername{PNE}}
\newcommand{\Fstrips}{\textsc{FSTRIPS}}
\newcommand{\FOL}{\textsc{FOL}}
\newcommand{\MPC}{\textsc{MPC}}
\newcommand{\TFD}{\propername{TFD}}
\newcommand{\AIBR}{\textsc{Aibr}}
\newcommand{\RRT}{\textsc{RRT}}
\newcommand{\SMTPlan}{\textsc{SMTPlan+}}


\newcommand{\Car}{\textsc{Car, Linear}}
\newcommand{\NLCar}{\textsc{Car, Nonlinear}}
\newcommand{\CarSC}{\textsc{Car, Linear, State Constraints}}
\newcommand{\NLCarSC}{\textsc{Car, Nonlinear, State Constraints}}
\newcommand{\Generator}{\textsc{Generator, Linear}}
\newcommand{\NLGenerator}{\textsc{Generator, Nonlinear}}
\newcommand{\Agile}{\textsc{Agile Robot}}
\newcommand{\Orbital}{\textsc{Orbital Rendezvous}}
\newcommand{\Descent}{\textsc{1D Powered Descent}}
\newcommand{\Intercept}{\textsc{Intercept}}
\newcommand{\Zermelo}{\textsc{Zermelo}}

% % formulas

\newcommand{\f}[1]{\sum_{r=0}^{m}\alpha_{{#1},t_0}^r e_{#1,t_0} + 
	\alpha_{#1,t_0}^m x_{#1}}
\newcommand{\ft}[2]{\alpha^m #1 + \sum_{r=0}^{m}\alpha^r (\sum_{i} w_i x_i + k)}
\newcommand{\ftm}[3]{\sum_{r=0}^{#3}\alpha_{{#1},#2}^r e_{#1,#2} + 
	\alpha_{#1,#2}^{#3} x_{#1}}

\newcommand{\eminus}{\sum_{j\neq i}w_j x^{i}_j + k}


\newcommand{\ftms}[3]{f_{#1}^{#2}(#3)}

\newcommand{\alphaf}[2]{\alpha_{{#1},#2}}

\newcommand{\pre}[1]{\ensuremath{\mathrm{pre}_{#1}}}
\newcommand{\eff}[1]{\ensuremath{\mathrm{eff}_{#1}}}
\newcommand{\action}[1]{\Tup{ \pre{#1}, \eff{#1} }}
\newcommand{\prop}[1]{{\cal P}_{A}}
\newcommand{\matr}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\invmatr}[1]{\mathbf{#1}^{-1}}
\newcommand{\transmatr}[1]{\mathbf{\Phi}(#1)}
\newcommand{\Matlab}{\propername{Matlab}}
\newcommand{\Octave}{\propername{Octave}}
\newcommand{\Sympy}{\propername{SymPy}}
\newcommand{\Mathematica}{\propername{Mathematica}}
\newcommand{\relproc}[2]{{\cal P}_{#1|x_{#2}}}
\newcommand{\MBP}{\propername{MBP}}
\newcommand{\OpTop}{\propername{OpTop}}
\newcommand{\Mode}[1]{{\cal M}(\matr{#1})}	
\newcommand{\ProcExpr}[2]{\xi_{x_{#1}|#2}(\matr{x})}
\newcommand{\Affected}[1]{\mathrm{aff}({#1})}
\newcommand{\Proc}[1]{\ensuremath{\mathrm{proc}(#1)}}
\newcommand{\Reals}{\ensuremath{\mathbb{R}}}

\newcommand{\Pong}{\textsc{Pong}}
\newcommand{\UCT}{\textsc{UCT}}
\newcommand{\BRFS}{\textsc{BrFS}}
\newcommand{\IW}[1]{\textsc{IW}$(#1)$}

\newcommand{\thereals}{\ensuremath{\mathbb{R}}}

\newcommand{\hzero}[1]{$s_{0}^{h_{#1}}$}
\newcommand{\hfinal}[1]{$s_{f}^{h_{#1}}$}
% Variants of the two macros above to be embedded in
% math mode
\newcommand{\mhzero}[1]{s_{0}^{h_{#1}}}
\newcommand{\mhfinal}[1]{s_{f}^{h_{#1}}}

\newcommand{\tzero}[1]{$T_{0}^{h_{#1}}$}
\newcommand{\tfinal}[1]{$T_{f}^{h_{#1}}$}
% Variants of the two macros above to be embedded in
% math mode
\newcommand{\mtzero}[1]{T_{0}^{h_{#1}}}
\newcommand{\mtfinal}[1]{T_{f}^{h_{#1}}}
\newcommand{\hinvar}[1]{${\cal I}^{h_{#1}}$}
\newcommand{\LP}{\propername{LP}}

\newcommand{\Rplus}{R^{+}}
\newcommand{\Rminus}{R^{-}}
\newcommand{\Vplus}{V^{+}}
\newcommand{\Vminus}{V^{-}}

\newcommand{\varmode}{\ensuremath{\textbf{ctl}}}
\newcommand{\litleft}{\ensuremath{\text{left}}}
\newcommand{\litstraight}{\ensuremath{\text{straight}}}
\newcommand{\litright}{\ensuremath{\text{right}}}

\newcommand{\rkfs}{\propername{FS+}$_{RK22}$}
\newcommand{\rkfsnv}{\propername{FS+}$_{RK22,NV}$}

\newcommand{\AStar}{\ensuremath{\text{A}^*}}

\sisetup{
	round-mode          = places, % Rounds numbers
	round-precision     = 2, % to 2 places
}

\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\VAL}{\propername{Val}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\matt}[1]{\ensuremath{\mathbf{#1}^{T}}}
\newcommand{\Useq}{\ensuremath{\mathbf{U}}}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\ubar}[1]{\text{\b{$#1$}}}

==> packages.tex <==
\usepackage{times}  %Required
\usepackage{helvet}  %Required
\usepackage{courier}  %Required
\usepackage{url}  %Required
\usepackage{graphicx}  %Required

\usepackage{enumitem} % Customized lists
\setlist[itemize]{noitemsep} % Make itemize lists more compact
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsthm}

\usepackage{latexsym}
\usepackage{enumerate}
\usepackage{mathtools}
\usepackage{url}
\usepackage{xspace}
\usepackage{soul}
\usepackage{todonotes}
%% for nice underlying \ul{xxx}
\setuldepth{x} 
%\usepackage{algorithm}
\usepackage{algorithmicx}
\usepackage[noend]{algpseudocode}
\usepackage{todonotes}
\usepackage{filecontents}
%\usepackage{stmaryrd}

% \renewcommand{\baselinestretch}{.99}
\usepackage{tikz}
\usepackage{pgf}
\usepackage{pgfplots}
\usepackage{longtable}
\usepackage{array}
\usepackage{colortbl}
\usepackage{booktabs} % For \toprule, \midrule and \bottomrule
\usepackage{siunitx} % Formats the units and values
\usepackage{pgfplotstable} % Generates table from .csv
%\usetikzlibrary{arrows,decorations,backgrounds,automata,shapes,patterns,decorations,backgrounds,plotmarks,calc,fit}
\usetikzlibrary{arrows,decorations,backgrounds,automata,shapes,patterns,decorations,backgrounds,plotmarks,calc,fit,positioning}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

==> pygment-settings.tex <==


\usepackage{fancyvrb}
\usepackage{color}



\makeatletter
\def\PY@reset{\let\PY@it=\relax \let\PY@bf=\relax%
    \let\PY@ul=\relax \let\PY@tc=\relax%
    \let\PY@bc=\relax \let\PY@ff=\relax}
\def\PY@tok#1{\csname PY@tok@#1\endcsname}
\def\PY@toks#1+{\ifx\relax#1\empty\else%
    \PY@tok{#1}\expandafter\PY@toks\fi}
\def\PY@do#1{\PY@bc{\PY@tc{\PY@ul{%
    \PY@it{\PY@bf{\PY@ff{#1}}}}}}}
\def\PY#1#2{\PY@reset\PY@toks#1+\relax+\PY@do{#2}}

%%%%
%% A colour scheme that follows (fairly close, but not exactly) the
%% ``white background'' palette on planning.domains:

%% keywords (:anything, define, domain, problem)
\expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}

%% ``builtins'' (operators etc)
\expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}

%% type names and typing hyphen
\expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.00}{##1}}}

%% variables (?var)
\expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.20,0.50,0.80}{##1}}}

%% integer and float constants
\expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}

%% comments
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.45,0.5,0.45}{##1}}}

%%%%
%% Below is the colour scheme we used originally for the book:

%% %% keywords (:anything, define, domain, problem)
%% \expandafter\def\csname PY@tok@k\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
%%
%% %% ``builtins'' (operators etc)
%% \expandafter\def\csname PY@tok@nb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
%%
%% %% type names and typing hyphen
%% \expandafter\def\csname PY@tok@nc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
%%
%% %% variables (?var)
%% \expandafter\def\csname PY@tok@nv\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
%%
%% %% integer and float constants
%% \expandafter\def\csname PY@tok@m\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
%% \expandafter\def\csname PY@tok@mi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
%% \expandafter\def\csname PY@tok@mf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
%%
%% %% comments
%% \expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}


%% other categories (not sure which are used)

\expandafter\def\csname PY@tok@gd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@gu\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.50,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@gt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.27,0.87}{##1}}}
\expandafter\def\csname PY@tok@gs\endcsname{\let\PY@bf=\textbf}
\expandafter\def\csname PY@tok@gr\endcsname{\def\PY@tc##1{\textcolor[rgb]{1.00,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@cm\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@vg\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@vi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@mh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@cs\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@ge\endcsname{\let\PY@it=\textit}
\expandafter\def\csname PY@tok@vc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@il\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@go\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.53,0.53}{##1}}}
\expandafter\def\csname PY@tok@cp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.74,0.48,0.00}{##1}}}
\expandafter\def\csname PY@tok@gi\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@gh\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@ni\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.60,0.60,0.60}{##1}}}
\expandafter\def\csname PY@tok@nl\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.63,0.63,0.00}{##1}}}
\expandafter\def\csname PY@tok@nn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@no\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.53,0.00,0.00}{##1}}}
\expandafter\def\csname PY@tok@na\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.49,0.56,0.16}{##1}}}
\expandafter\def\csname PY@tok@nd\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@ne\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.82,0.25,0.23}{##1}}}
\expandafter\def\csname PY@tok@nf\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,1.00}{##1}}}
\expandafter\def\csname PY@tok@si\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@s2\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@nt\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s1\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ch\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@gp\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.00,0.50}{##1}}}
\expandafter\def\csname PY@tok@sh\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@ow\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.67,0.13,1.00}{##1}}}
\expandafter\def\csname PY@tok@sx\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@bp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c1\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@o\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kc\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@c\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@err\endcsname{\def\PY@bc##1{\setlength{\fboxsep}{0pt}\fcolorbox[rgb]{1.00,0.00,0.00}{1,1,1}{\strut ##1}}}
\expandafter\def\csname PY@tok@mb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@ss\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.10,0.09,0.49}{##1}}}
\expandafter\def\csname PY@tok@sr\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.53}{##1}}}
\expandafter\def\csname PY@tok@mo\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.40,0.40,0.40}{##1}}}
\expandafter\def\csname PY@tok@kd\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@kn\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@cpf\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.25,0.50,0.50}{##1}}}
\expandafter\def\csname PY@tok@kr\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@s\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@kp\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.00,0.50,0.00}{##1}}}
\expandafter\def\csname PY@tok@w\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.73,0.73}{##1}}}
\expandafter\def\csname PY@tok@kt\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.69,0.00,0.25}{##1}}}
\expandafter\def\csname PY@tok@sc\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@sb\endcsname{\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}
\expandafter\def\csname PY@tok@se\endcsname{\let\PY@bf=\textbf\def\PY@tc##1{\textcolor[rgb]{0.73,0.40,0.13}{##1}}}
\expandafter\def\csname PY@tok@sd\endcsname{\let\PY@it=\textit\def\PY@tc##1{\textcolor[rgb]{0.73,0.13,0.13}{##1}}}

\def\PYZbs{\char`\\}
\def\PYZus{\char`\_}
\def\PYZob{\char`\{}
\def\PYZcb{\char`\}}
\def\PYZca{\char`\^}
\def\PYZam{\char`\&}
\def\PYZlt{\char`\<}
\def\PYZgt{\char`\>}
\def\PYZsh{\char`\#}
\def\PYZpc{\char`\%}
\def\PYZdl{\char`\$}
\def\PYZhy{\char`\-}
\def\PYZsq{\char`\'}
\def\PYZdq{\char`\"}
\def\PYZti{\char`\~}
% for compatibility with earlier versions
\def\PYZat{@}
\def\PYZlb{[}
\def\PYZrb{]}
\makeatother

